Dataset Bias in Android Malware Detection

Researchers have proposed kinds of malware detection methods to solve the explosive mobile security threats. We argue that the experiment results are inflated due to the research bias introduced by the variability of malware dataset. We explore the impact of bias in Android malware detection in three aspects, the method used to flag the ground truth, the distribution of malware families in the dataset, and the methods to use the dataset. We implement a set of experiments of different VT thresholds and find that the methods used to flag the malware data affect the malware detection performance directly. We further compare the impact of malware family types and composition on malware detection in detail. The superiority of each approach is different under various combinations of malware families. Through our extensive experiments, we showed that the methods to use the dataset can have a misleading impact on evaluation, and the performance difference can be up to over 40%. We argue that these research biases observed in this paper should be carefully controlled/eliminated to enforce a fair comparison of malware detection techniques. Providing reasonable and explainable results is better than only reporting a high detection accuracy with vague dataset and experimental settings.

==> 06-RQ3.tex <==
\section{The Impact of Mobile Adware}

\label{subsection:adware}
\subsection{The Construction of Malware Set}

To evaluate the impact of mobile adware, we perform a comparative experiment with RQ1. 
Similar to RQ1, we also extract 23 groups of malware from our dataset. Each group contains 1,000 malware apks with a different VT number. The VT numbers range from 1 to 20 in different groups, with three additional groups of \emph{From 21 to 25}, \emph{From 26 to 30} and \emph{More than 31} .

For each group, the 1,000 malware apks consist of 500 non-ad malware apks and 500 adware apks.
We recall that all the malware in RQ1 are non-adware, thus we can evaluate the impact of adware by comparing the results between the experiment in RQ3 and RQ1.

\subsection{Result of RQ3}

The results of RQ3 is shown in Figure \ref{fig:rq3}. In each chart, there are two lines in different colors: The blue line represents the accurary of full no-ad malware in different threshold, taking advantage of the experiment result in RQ1; the orange line represents the accurary of half adware, half no-ad malware.

The average accurary for the two lines in 92.9\%, 93.7\% and 88.8\%, 88.5\% and 84.2\%, 82.4\% respectively for csbd, drebin and mamadroid. Under the same threshold, the average difference between full non-ad malware and half adware is 2.29\%, 2.01\% and 2.02\% respectively. We could see from \ref{fig:rq3-recall} that the recall of almost all algorithms has great changes, so adware is still a challenge for the current algorithms.
 In particular, mamadroid is sensitive to whether adware is considered as malware. Accuracy, precision and recall of mamadroid change greatly, and it is greatly affected by the dataset bias.


% RQ3 shows that, under the same VT threshold, the impact of mobile adware on the malware detection is limited.

\begin{tcolorbox}[title= \textbf{RQ-3} Answer, left=2pt, right=2pt, top=2pt,bottom=2pt]
Whether adware is contained in the dataset will affect the malware detection performance in a certain extent. Different algorithms have different sensitivity to whether adware is included in the dataset. The comparison of malware detection performance between algorithms is closely related to the construction of datasets.
% Under the same VT threshold, the impact of mobile adware on the malware detection is limited. The average difference between full non-ad malware and half adware is no more than 3\%. The influence of mobile adware can be ignored to some extent.
\end{tcolorbox}

\begin{figure}[tp]
\centering
\subfigure[Accuracy with and without adware]
{
\includegraphics[width=0.32\linewidth]{Image/csbd-Adware-Accuracy.png}
\includegraphics[width=0.32\linewidth]{Image/drebin-Adware-Accuracy.png}
\includegraphics[width=0.32\linewidth]{Image/mamadroid-Adware-Accuracy.png}
\label{fig:rq3}
}
\subfigure[Precision with and without adware]
{
\includegraphics[width=0.32\linewidth]{Image/csbd-Adware-Precision.png}
\includegraphics[width=0.32\linewidth]{Image/drebin-Adware-Precision.png}
\includegraphics[width=0.32\linewidth]{Image/mamadroid-Adware-Precision.png}
\label{fig:rq3-precision}
}
\subfigure[The recall with and without adware]
{
\includegraphics[width=0.32\linewidth]{Image/csbd-Adware-Recall.png}
\includegraphics[width=0.32\linewidth]{Image/drebin-Adware-Recall.png}
\includegraphics[width=0.32\linewidth]{Image/mamadroid-Adware-Recall.png}
\label{fig:rq3-recall}
}

\caption{The impact of mobile adware.}
\end{figure}

% compare wrong
% \begin{figure*}[htbp]
% \centering
% \subfigure[Accuracy with imbalanced distribution of csbd]
% {	\label{fig:rq3-csbdAccuracy}
% 	\includegraphics[width=0.31\linewidth]{Image/cmpBalanceCsbd.png}

% }
% \subfigure[Accuracy with imbalanced distribution of drebin]
% {
% 	\label{fig:rq3-csbdPrecision}
% 	\includegraphics[width=0.31\linewidth]{Image/cmpBalanceDrebin.png}
% }
% \subfigure[Accuracy with imbalanced distribution of mamadroid]
% {
% 	\label{fig:rq3-csbdRecall}
% 	\includegraphics[width=0.31\linewidth]{Image/cmpBalanceMamadroid.png}
% }

% \caption{RQ3 Accuracy with imbalanced distribution}
% \label{fig:rq4}
% \end{figure*}


% \begin{figure}[tp]
% \centering
% \includegraphics[width=\linewidth]{Image/cmpBalanceCsbd.png}
% \caption{Accuracy with imbalanced distribution of csbd}
% \label{fig:rq3-recall}
% \end{figure}

% \begin{figure}[tp]
% \centering
% \includegraphics[width=\linewidth]{Image/cmpBalanceDrebin.png}
% \caption{Accuracy with imbalanced distribution of drebin}
% \label{fig:rq3-recall}
% \end{figure}

% \begin{figure}[tp]
% \centering
% \includegraphics[width=\linewidth]{Image/cmpBalanceMamadroid.png}
% \caption{Accuracy with imbalanced distribution of mamadroid}
% \label{fig:rq3-recall}
% \end{figure}


==> macros.tex <==
%\usepackage{times}
\usepackage{graphicx}
%\usepackage{epsf}
%\usepackage{verbatim}
%\usepackage{psfig}
%\usepackage{cite}
%\usepackage{wrapfig}
%\usepackage{xcolor}
\usepackage{mdwlist}
\usepackage{multirow}
\usepackage{subfig}
\usepackage{float}
\usepackage{adjustbox}
\usepackage{url}
\usepackage{color}
\usepackage{alltt}
\usepackage{xspace}
\usepackage[ruled,linesnumbered]{algorithm2e}
\newcommand\mycommfont[1]{\scriptsize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}

\SetKwInput{KwInput}{Input}
\SetKwInput{KwOutput}{Output}
\SetKwProg{Fn}{Function}{}{end}

\usepackage{hyperref} %change this later
\hypersetup{
    citebordercolor={0 1 0},
    citecolor=blue,
    colorlinks=false,
    filebordercolor={0 .5 .5},
    filecolor=green,
    linkbordercolor={1 0 0},
    linkcolor=blue,
    menubordercolor={1 0 0},
    pageanchor=true,
    pagebackref=true,
    pdfborder={0 0 1},
    pdfpagelabels=true,
    pdftex,
    plainpages=false,
    urlbordercolor={0 1 1},
    urlcolor=blue,
}
\usepackage{syntax}
\usepackage{multicol}
%\usepackage{newfloat}
\usepackage{wrapfig}
\usepackage{float}

\newcommand{\revision}[2]{
	{\color{red} #1} :
	{\color{blue} #2}
}



\newcommand{\Fix}[1]{{\large\textbf{FIX}}#1{\large\textbf{FIX}}}
%\newcommand{\Fix}[1]{#1}
\newcommand{\New}[1]{{\large\textbf{New}}#1{\large\textbf{New}}}
\newcommand{\FixResolved}[1]{#1}
\newcommand{\realprojects}{a real project}
\newcommand{\Add}{\CodeIn{add}}
\newcommand{\AVTree}{\CodeIn{AVTree}}
\newcommand{\Assignment}[3]{$\langle$ \Object{#1}, \Object{#2}, \Object{#3} $\rangle$}
\newcommand{\BinaryTreeRemove}{\CodeIn{BinaryTree\_remove}}
\newcommand{\BinaryTree}{\CodeIn{BinaryTree}}
\newcommand{\Caption}{\caption}
\newcommand{\Char}[1]{`#1'}
\newcommand{\CheckRep}{\CodeIn{checkRep}}
\newcommand{\ClassC}{\CodeIn{C}}
\newcommand{\CodeIn}[1]{{\small\texttt{#1}}}
\newcommand{\CodeOutSize}{\scriptsize}
\newcommand{\Comment}[1]{}
\newcommand{\Ensures}{\CodeIn{ensures}}
\newcommand{\ExtractMax}{\CodeIn{extractMax}}
\newcommand{\FAL}{field-ordering}
\newcommand{\FALs}{field-orderings}
\newcommand{\Fact}{observation}
\newcommand{\Get}{\CodeIn{get}}
\newcommand{\HashSet}{\CodeIn{HashSet}}
\newcommand{\HeapArray}{\CodeIn{HeapArray}}
\newcommand{\Intro}[1]{\emph{#1}}
\newcommand{\Invariant}{\CodeIn{invariant}}
\newcommand{\JUC}{\CodeIn{java.\-util.\-Collections}}
\newcommand{\JUS}{\CodeIn{java.\-util.\-Set}}
\newcommand{\JUTM}{\CodeIn{java.\-util.\-TreeMap}}
\newcommand{\JUTS}{\CodeIn{java.\-util.\-TreeSet}}
\newcommand{\JUV}{\CodeIn{java.\-util.\-Vector}}
\newcommand{\JMLPlusJUnit}{JML+JUnit}
\newcommand{\Korat}{Korat}
\newcommand{\Left}{\CodeIn{left}}
\newcommand{\Lookup}{\CodeIn{lookup}}
\newcommand{\MethM}{\CodeIn{m}}
\newcommand{\Node}[1]{\CodeIn{N}$_#1$}
\newcommand{\Null}{\CodeIn{null}}
\newcommand{\Object}[1]{\CodeIn{o}\ensuremath{_#1}}
\newcommand{\PostM}{\MethM$_{post}$}
\newcommand{\PreM}{\MethM$_{pre}$}
\newcommand{\Put}{\CodeIn{put}}
\newcommand{\Remove}{\CodeIn{remove}}
\newcommand{\RepOk}{\CodeIn{repOk}}
\newcommand{\Requires}{\CodeIn{requires}}
\newcommand{\Reverse}{\CodeIn{reverse}}
\newcommand{\Right}{\CodeIn{right}}
\newcommand{\Root}{\CodeIn{root}}
\newcommand{\Set}{\CodeIn{set}}
\newcommand{\State}[1]{2^{#1}}
\newcommand{\TestEra}{TestEra}
\newcommand{\TreeMap}{\CodeIn{TreeMap}}
\newcommand{\smoot}{\textsf{MSeqGen} \xspace}

%\newenvironment{CodeOut}{\begin{scriptsize}}{\end{scriptsize}}
\newenvironment{CodeOut}{\begin{small}}{\end{small}}
\newenvironment{SmallOut}{\begin{small}}{\end{small}}

\newcommand{\pairwiseEquals}{PairwiseEquals}
\newcommand{\monitorEquals}{MonitorEquals}
%\newcommand{\monitorWField}{WholeStateW}
\newcommand{\traverseField}{WholeState}
\newcommand{\monitorSMSeq}{ModifyingSeq}
\newcommand{\monitorSeq}{WholeSeq}

\newcommand{\IntStack}{\CodeIn{IntStack}}
\newcommand{\UBStack}{\CodeIn{UBStack}}
\newcommand{\BSet}{\CodeIn{BSet}}
\newcommand{\BBag}{\CodeIn{BBag}}
\newcommand{\ShoppingCart}{\CodeIn{ShoppingCart}}
\newcommand{\BankAccount}{\CodeIn{BankAccount}}
\newcommand{\BinarySearchTree}{\CodeIn{BinarySearchTree}}
\newcommand{\LinkedList}{\CodeIn{LinkedList}}

\newcommand{\Book}{\CodeIn{Book}}
\newcommand{\Library}{\CodeIn{Library}}

\newcommand{\Jtest}{Jtest}
\newcommand{\JCrasher}{JCrasher}
\newcommand{\Daikon}{Daikon}
\newcommand{\JUnit}{JUnit}

\newcommand{\trie}{trie}

\newcommand{\Perl}{Perl}


\newcommand{\SubjectCount}{11}
\newcommand{\DSSubjectCount}{two}

\newcommand{\Equals}{\CodeIn{equals}}
\newcommand{\Pairwise}{PairwiseEquals}
\newcommand{\Subgraph}{MonitorEquals}
\newcommand{\Concrete}{WholeState}
\newcommand{\ModSeq}{ModifyingSeq}
\newcommand{\Seq}{WholeSeq}
\newcommand{\Aeq}{equality}

\newcommand{\Meaning}[1]{\ensuremath{[\![}#1\ensuremath{]\!]}}
\newcommand{\Pair}[2]{\ensuremath{\langle #1, #2 \rangle}}
\newcommand{\Triple}[3]{\ensuremath{\langle #1, #2, #3 \rangle}}
\newcommand{\SetSuch}[2]{\ensuremath{\{ #1 | #2 \}}}
\newcommand{\Equiv}[2]{\ensuremath{#1 \EquivSTRel{} #2}}
\newcommand{\EquivME}{\Equiv}
\newcommand{\EquivST}{\Equiv}
\newcommand{\EquivSTRel}{\ensuremath{\cong}}
\newcommand{\Redundant}[2]{\ensuremath{#1 \lhd #2}}
\newcommand{\VB}{\ensuremath{\mid}}
\newcommand{\MES}{method-entry state}
\newtheorem{definition}{Definition}

\newcommand{\SmallSpace}{\vspace*{-1.5ex}}
\newcommand{\Item}{\SmallSpace\item}
\newenvironment{Itemize}{\begin{itemize}}{\end{itemize}\SmallSpace}
\newenvironment{Enumerate}{\begin{enumerate}}{\end{enumerate}\SmallSpace}


\newcommand{\CenterCell}[1]{\multicolumn{1}{c|}{#1}}



%%%
\newcommand{\red}[1]{{-\textcolor{red}{#1}-}}
\newcommand{\pgao}[1]{-\textcolor{red}{(PG: #1)-}}

\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\myparatight}[1]{\vspace*{0.5ex}\noindent\emph{\small \textbf{#1}}:}
%\newcommand{\myparatight}[1]{\noindent{\bf {#1}:}}
\newcommand{\norm}[1]{\left\lVert #1 \right\rVert_1}
\newcommand{\sign}{sign}
\newcommand{\eat}[1]{}

%\DeclareFloatingEnvironment[
%  % the file extension for the file used to create the list:
%  fileext   = logr,% don't use log here!
%  % the heading for the list:
%  listname  = {List of Grammars},
%  % the name used in captions:
%  name      = Grammar,
%  % the default floating parameters if the environment is used
%  % without optional argument:
%  placement = !htbp
%]{BNF}

\usepackage[font=footnotesize]{caption}
\captionsetup[figure]{font=bf,skip=0pt}%set figure caption
\captionsetup[table]{font=bf,skip=0pt}%set table caption
\newcommand{\distance}{2pt}
\setlength{\textfloatsep}{\distance}%set distance between figure/tables on the top/bottom with text
\setlength{\floatsep}{\distance}%set distance between figures or tables
\setlength{\intextsep}{\distance}%set distance between figures/tables in text with text
\setlength{\dbltextfloatsep}{\distance} %distance between a figure/table spanning both columns and the text;
\setlength{\dblfloatsep}{\distance} %distance between two figures/tables spanning both columns.

\usepackage{listings}
\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
%\definecolor{mymauve}{rgb}{0.58,0,0.82}
\renewcommand{\ttdefault}{pcr}
%\renewcommand{\lstlistingname}{Code Snippet}

\lstset{
	backgroundcolor=\color{white},
	basicstyle=\scriptsize\ttfamily\bfseries,
	breaklines=true,
	keepspaces=true,
	numbers=left,
	numbersep=4pt,
	numberstyle=\tiny\color{gray},
	rulecolor=\color{black},
	showspaces=false,
	showstringspaces=false,
	showtabs=false,
	stepnumber=1,
	stringstyle=\color{black},
	tabsize=2,
	language=java
}
\lstset{
	commentstyle=\color{mygreen},
	%	frame=lines,
	keywordstyle=\color{blue},
	%	keywordstyle=[2]\color{blue},
	morekeywords={ImageView,R,Button, ImageButton,EditText,LinearLayout,TextView,RelativeLayout,ListView,selector,item}, % no space
	%	keywords=[2] {proc,file,ip}
}

\newcommand{\incode}[1]{\lstinline{#1}}

\newcommand{\eg}{e.g., }
\newcommand{\ie}{i.e., }
\newcommand{\etal}{et al. }




\newcommand{\whyper}{\textsc{Whyper}\xspace}
\newcommand{\DI}{\textsc{$\Delta$Infer}\xspace}
\newcommand {\cilppa} {{\textsc{Arc++}}\xspace}
\newcommand {\appcontext} {{\textsc{AppContext}}\xspace}
\newcommand {\supor} {{\textsc{Supor}}\xspace}
\newcommand {\tg} {{\textsc{TGMiner}}\xspace}
\newcommand {\tp} {{\textsc{Text2Policy}}\xspace}
\newcommand {\covana} {{\textsc{Covana}}\xspace}
\newcommand {\tbql} {{\textsc{Tbql}}\xspace}
\newcommand {\tool} {{\textsc{IconIntent}}\xspace}


